Medical Image Registration via Neural Fields

Image registration is an essential step in many medical image analysis tasks. Traditional methods for image registration are primarily optimization-driven, finding the optimal deformations that maximize the similarity between two images. Recent learning-based methods, trained to directly predict transformations between two images, run much faster, but suffer from performance deficiencies due to model generalization and the inefficiency in handling individual image specific deformations. Here we present a new neural net based image registration framework, called NIR (Neural Image Registration), which is based on optimization but utilizes deep neural nets to model deformations between image pairs. NIR represents the transformation between two images with a continuous function implemented via neural fields, receiving a 3D coordinate as input and outputting the corresponding deformation vector. NIR provides two ways of generating deformation field: directly output a displacement vector field for general deformable registration, or output a velocity vector field and integrate the velocity field to derive the deformation field for diffeomorphic image registration. The optimal registration is discovered by updating the parameters of the neural field via stochastic gradient descent. We describe several design choices that facilitate model optimization, including coordinate encoding, sinusoidal activation, coordinate sampling, and intensity sampling. Experiments on two 3D MR brain scan datasets demonstrate that NIR yields state-of-the-art performance in terms of both registration accuracy and regularity, while running significantly faster than traditional optimization-based methods.

==> figs/cs_performance_plot.tex <==
\begin{figure}
\centering
\includegraphics[width=0.5\textwidth]{imgs/cs_performance_radar.png}
\vspace{-1em}
\caption{\textbf{Comparison of registration performance applying different coordinate samplers}.}
\label{fig:cs_performance_comparison}
\end{figure}

==> latexmkrc <==
# --- This file allows you to quickly change the style in case you need to resubmit
$ENV{'TEXINPUTS'}='./cvpr22//:' . $ENV{'TEXINPUTS'}; 
$ENV{'BSTINPUTS'}='./cvpr22//:' . $ENV{'BSTINPUTS'};

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> sec/4_6_experiments_with_nodeo.tex <==
\subsection{Comparisons with NODEO}
\label{subsec:results_comp_nodeo}

NODEO\cite{wu2022nodeo} is singled out to be compared against because it is the most similar work with ours. Same as us, they also propose to obtain the deformation field by integrating the neural velocity field via neural ODE. 
%%
It seems to be quite similar to our NIR-D-Diff, but there are many differences. The most fundamental difference between theirs and ours lies in the network architectures. Their neural velocity field is basically a Unet-like 3D CNN model with fully connected bottleneck layers, whereas ours is an all-MLP network with coordinate encoding and sinusoidal activation functions. During optimization, NODEO receives the whole grid coordinates as input and predicts the entire deformations in every iteration. For the sake of memory efficiency, NODEO must reduce the spatial size or the channel number of the feature maps, which may make it difficult for the neural network to represent the high-resolution deformation fields.
%%
More importantly, since NODEO architecture incorporates 3D convolutional layers, it is difficult to achieve their objective to predict the time-invariant velocity field for the 3D medical picture registration experiment. 
Suppose the predicted velocity vector of one coordinate is $\overrightarrow{0}$ while those of its neighboring coordinates are not $\overrightarrow{0}$, the output of that coordinate in the next-step evaluation of the dynamic function should be $\overrightarrow{0}$ according to the definition of the stationary velocity field, but it is nearly impossible since the output of 3D CNN is not invariant to the deformed neighborhood. We believe this is one of the reasons why they need to enforce smoothness constraints to the predicted velocity fields. 

\input{tabs/comparison_with_nodeo}
They haven't released their official implementations yet and some technique details are missing in their paper, thus we can only copy their reported registration performance on OASIS image pairs from their paper. 
%%
For a fair comparison with NODEO in experiment (2), we apply the data split, data source and data processing, the same as what NODEO used.
%%
In addition, our performance listed in Tab.~\ref{tab:comp_with_nodeo} is generated from the NIR-D-Diff model optimized for 100 iterations, which takes about 65s, less than what NODEO takes to achieve their reported performance. 
As can be seen from Tab.~\ref{tab:comp_with_nodeo}, with less GPU memory consumption for optimization, less optimization time as well as less regularization, our NIR-D-Diff can outperform NODEO in $\displaystyle DSC_v$ by 0.2 larger and in $\mathbf{J}_{\leq 0}~(\downarrow)$ by over 80x smaller. 

==> tabs/comparison_with_nodeo.tex <==
\begin{table}[!ht]
\centering
\caption{
\textbf{Registration Performance Comparison between MIRNF-D-Diff and NODEO on Experiment (2). The $\displaystyle DSC_v$ below is the average volumetric Dice's Coefficients of 28 anatomical structures, following the setting of NODEO} 
}
\begin{tabular}{lcccc}
\toprule
\multirow{2}{*}{Method}          & \multirow{2}{*}{$\displaystyle DSC_v~(\uparrow)$}          & \multirow{2}{*}{$\mathbf{J}_{\leq 0}~(\downarrow)$}    & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Memory\\ (MB) \end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Time\\ (s) \end{tabular}}           \\
& & & \\ \midrule
NODEO           & 0.779              & 3e-04        & 3863      &$\approx$80       \\
MIRNF-D-Diff    & \textbf{??}    & \textbf{??}     & \textbf{3177}     &\textbf{$\approx$65}         \\ \bottomrule
\end{tabular}
\label{tab:comp_with_nodeo}
\end{table}

==> tabs/effectiveness_of_nfs.tex <==



==> tabs/time_vs_performance.tex <==
\begin{table}[]
\begin{tabular}{lcccccccc}
\hline
Metrics            & \multicolumn{4}{c}{DSC}                                & \multicolumn{4}{c}{njdet}                  \\ \hline
Method / Iteration & 100    & 300    & 600    & \multicolumn{1}{c|}{900}    & 100      & 300      & 600      & 900       \\ \hline
MIRNF-D-Diff       & 0.7989 & 0.8093 & 0.8104 & \multicolumn{1}{c|}{0.8107} & 2.40e-06 & 4.03e-05 & 1.12e-04 & 1.79e-04  \\
MIRNF-P-Diff       & 0.7071 & 0.7656 & 0.7931 & \multicolumn{1}{c|}{0.8059} & 0        & 8.43e-08 & 2.01e-06 & 3..72e-06 \\ \hline
MIRNF-H-Diff       & 0.8012 & 0.8083 & 0.8105 & \multicolumn{1}{c|}{0.8117} & 2.97e-06 & 1.30e-06 & 1.22e-06 & 2.96e-06  \\ \hline
\end{tabular}
\end{table}
